LLVM Translation Validation Automated with Large Language Models and Lean

LLVM is the cornerstone of modern compilers, but its subtle intermediate representation (IR) semantics make transformations error-prone and necessitate formal verification. Alive2, a state-of-the-art translation validator based on satisfiability modulo theories, has achieved substantial success in automating the validation of LLVM transformations. However, it still faces scalability limitations, does not support symbolic bitwidths, and offers only bounded guarantees for loops. In contrast, interactive theorem provers such as Lean can address these cases but require substantial proof engineering. In this paper, we present Trivet, a framework combining large language models (LLMs) and Lean for automated translation validation of LLVM transformations. Trivet generates structured proof scaffolds based on source and target functions, automatically discharges obligations amenable to deterministic reasoning, and delegates transformationspecific obligations to LLMs. It produces refinement proofs or counterexample-based refutations, with every successful verdict checked by the Lean kernel. On 148 LLVM transformations, Trivet verifies or refutes 147, leaving one invalid case unresolved. Successful cases include 60 loop-free transformations with symbolic bitwidths, 27 cases from a restricted class of loop-containing transformations, and 10 complex valid fixed-bitwidth cases on which Alive2 times out. Compared with an unscaffolded baseline, scaffolding enables 26 additional proofs. On cases solved by both configurations, it reduces mean proof time by 75.9% and mean monetary cost by 88%.

==> constants.tex <==
\RequirePackage{xfp}

\newcommand{\proj}{\projectname{Trivet}}
\newcommand{\projminus}{\ensuremath{\proj^{-}}\xspace}
\newcommand{\llm}{LLM\xspace}
\newcommand{\llms}{LLMs\xspace}
\newcommand{\llvm}{LLVM\xspace}
\newcommand{\mlir}{MLIR\xspace}
\newcommand{\ir}{IR\xspace}
\newcommand{\ub}{UB\xspace}

\newcommand{\smt}{SMT\xspace}
\newcommand{\itp}{ITP\xspace}
\newcommand{\itps}{ITPs\xspace}
\newcommand{\alivetwo}{Alive2\xspace}
\newcommand{\vellvm}{Vellvm\xspace}
\newcommand{\leanmlir}{Lean-MLIR\xspace}
\newcommand{\coq}{Rocq\xspace}
\newcommand{\lean}{Lean\xspace}

\newcommand{\instcombine}{InstCombine\xspace}
\newcommand{\instCombineCodeSize}{50,000\xspace}

\newcommand{\GuardRuleCount}{nine\xspace}

\newcommand{\ph}[1]{\textcolor{red}{\textbf{[#1]}}\xspace}

\newcommand{\ValBenchCount}{%
  \AblLoopCalc{0}{\ValBenchCountloopfree+\ValBenchCountloop}}
\newcommand{\ValBenchCountFixed}{%
  \AblLoopCalc{0}{\DsFix+\DsMutFix+\ValLoopValidFixCount+\ValLoopInvalidFixCount}}
\newcommand{\ValBenchCountSymbolic}{%
  \AblLoopCalc{0}{\DsSym+\DsMutSym+\ValLoopValidSymCount+\ValLoopInvalidSymCount}}
\newcommand{\ValBenchCountloop}{%
  \AblLoopCalc{0}{\ValLoopValidCount+\ValLoopInvalidCount}}
\newcommand{\ValBenchCountloopfree}{\AblLoopCalc{0}{\DsTotal+\DsMut}}

\newcommand{\ValVerifiedCount}{\AblLoopCalc{0}{\RqOneVerified+\ValLoopCount}}
\newcommand{\ValRefutedCount}{%
  \AblLoopCalc{0}{\RqTwoRefuted+\RqThreeInvalidSymRefuted+\RqThreeInvalidFixRefuted}}
\newcommand{\ValFixedBWTimeoutCount}{10\xspace}
\newcommand{\ValParamBWCount}{\RqOneSymVerified} %

\newcommand{\ValLoopCount}{%
  \AblLoopCalc{0}{\RqThreeValidSymProved+\RqThreeValidFixProved}}
\newcommand{\ValSolvedCount}{%
  \AblLoopCalc{0}{\ValVerifiedCount+\ValRefutedCount}}
\newcommand{\ValParamBWSolvedCount}{%
  \AblLoopCalc{0}{\ValParamBWCount+\RqTwoSymRefuted}}
\newcommand{\ValLoopSolvedCount}{%
  \AblLoopCalc{0}{\ValLoopCount+\RqThreeInvalidSymRefuted+\RqThreeInvalidFixRefuted}}
\newcommand{\ValLoopValidCount}{\RqThreeValidCaseCount}
\newcommand{\ValLoopValidFixCount}{\RqThreeValidCaseCountFixed}
\newcommand{\ValLoopValidSymCount}{\RqThreeValidCaseCountSymbolic}

\newcommand{\ValLoopInvalidCount}{\RqThreeInvalidCaseCount}
\newcommand{\ValLoopInvalidFixCount}{\RqThreeInvalidCaseCountFixed}
\newcommand{\ValLoopInvalidSymCount}{\RqThreeInvalidCaseCountSymbolic}

\newcommand{\ValScaffoldWallTimeReduction}{%
  \AblLoopCalc{1}{100*(1-
    (\AblPairScafSecondsRaw+\AblCexPairScafSecondsRaw
      +\AblLoopPairScafMean*\AblLoopPairCount
      +\AblLoopCexPairScafMean*\AblLoopCexPairCount)/
    (\AblPairBaseSecondsRaw+\AblCexPairBaseSecondsRaw
      +\AblLoopPairBaseMean*\AblLoopPairCount
      +\AblLoopCexPairBaseMean*\AblLoopCexPairCount))}\unskip\%\xspace}
\newcommand{\ValScaffoldCostReduction}{88\%\xspace}
\newcommand{\ValScaffoldNewSolveCount}{%
  \AblLoopCalc{0}{\AblOnlyScafTotalRaw
    +\AblLoopScafSolved-\AblLoopBaseSolved
    +\AblLoopCexScafRefuted-\AblLoopCexBaseRefuted}}
\newcommand{\AliveFixedBWVerifiedCount}{20\xspace}
\newcommand{\AliveFixedBWCount}{30\xspace}       %

\newcommand{\precondition}{\ensuremath{\mathit{PRE}}\xspace}
\newcommand{\lhs}{\ensuremath{\mathit{LHS}}\xspace}
\newcommand{\rhs}{\ensuremath{\mathit{RHS}}\xspace}
\newcommand{\src}{\ensuremath{\mathit{src}}\xspace}
\newcommand{\tgt}{\ensuremath{\mathit{tgt}}\xspace}
\newcommand{\refine}[2]{\ensuremath{#1 \sqsupseteq #2}\xspace}
\newcommand{\poweroftwo}{\ensuremath{\mathsf{PowerOfTwo}}}

\newcommand{\rqone}{RQ1\xspace}
\newcommand{\rqtwo}{RQ2\xspace}
\newcommand{\rqthree}{RQ3\xspace}
\newcommand{\rqfour}{RQ4\xspace}
\newcommand{\rqoneContent}{Can \proj effectively validate real-world valid LLVM transformations?}
\newcommand{\rqtwoContent}{Can \proj effectively refute real-world invalid LLVM transformations?}
\newcommand{\rqthreeContent}{Can \proj effectively validate and refute loop-containing LLVM transformations derived from real-world cases?}
\newcommand{\rqfourContent}{What is the impact of \proj's scaffold on refinement and counterexample proof generation?}

\newcommand{\exptime}{two hours\xspace}


\newcommand{\DsTotal}{60\xspace}
\newcommand{\DsSym}{30\xspace}
\newcommand{\DsFix}{30\xspace}
\newcommand{\DsFs}{15\xspace}                 %
\newcommand{\DsFt}{15\xspace}                 %
\newcommand{\DsMut}{60\xspace}                %
\newcommand{\DsMutSym}{30\xspace}
\newcommand{\DsMutFix}{30\xspace}
\newcommand{\DsMutFs}{15\xspace}
\newcommand{\DsMutFt}{15\xspace}

\newcommand{\RqOneCount}{60\xspace}
\newcommand{\RqOneVerified}{60\xspace}
\newcommand{\RqOneMedian}{522\xspace}
\newcommand{\RqOneMean}{684\xspace}
\newcommand{\RqOneSymCount}{30\xspace}
\newcommand{\RqOneSymVerified}{30\xspace}
\newcommand{\RqOneSymMedian}{614\xspace}
\newcommand{\RqOneSymMean}{722\xspace}
\newcommand{\RqOneFixCount}{30\xspace}
\newcommand{\RqOneFixVerified}{30\xspace}
\newcommand{\RqOneFixMean}{647\xspace}
\newcommand{\RqOneFsMedian}{463\xspace}
\newcommand{\RqOneFsMean}{487\xspace}

\newcommand{\AliveFtVerified}{5\xspace}
\newcommand{\AliveFtMedian}{941\xspace}       %
\newcommand{\AliveFtMean}{823\xspace}         %
\newcommand{\AliveFixedBWMean}{206\xspace}    %
\newcommand{\AliveFixedBWTimeoutCount}{10\xspace} %

\newcommand{\RqTwoCount}{60\xspace}
\newcommand{\RqTwoRefuted}{60\xspace}
\newcommand{\RqTwoMean}{61\xspace}
\newcommand{\RqTwoFixCount}{30\xspace}
\newcommand{\RqTwoFixRefuted}{30\xspace}
\newcommand{\RqTwoFixMean}{56\xspace}
\newcommand{\RqTwoFixMedian}{46\xspace}
\newcommand{\RqTwoFixMin}{31\xspace}
\newcommand{\RqTwoFixMax}{210\xspace}
\newcommand{\RqTwoSymCount}{30\xspace}
\newcommand{\RqTwoSymRefuted}{30\xspace}
\newcommand{\RqTwoSymMean}{66\xspace}
\newcommand{\RqTwoSymMedian}{56\xspace}
\newcommand{\RqTwoSymMin}{32\xspace}
\newcommand{\RqTwoSymMax}{204\xspace}

\newcommand{\RqTwoProposeMean}{47\xspace}
\newcommand{\RqTwoCertifyMean}{14\xspace}
\newcommand{\RqTwoProposeShare}{77\%\xspace}
\newcommand{\RqTwoCertifyShare}{23\%\xspace}

\newcommand{\AliveCexCount}{30\xspace}
\newcommand{\AliveCexRefuted}{29\xspace}
\newcommand{\AliveCexMean}{47\xspace}
\newcommand{\AliveCexMin}{0.08\xspace}
\newcommand{\AliveCexMax}{1023\xspace}
\newcommand{\AliveCexMedian}{0.103\xspace}

\newcommand{\RqThreeEvaluatedCount}{%
  \AblLoopCalc{0}{\RqThreeValidCaseCount+\RqThreeInvalidCaseCount}}

\newcommand{\RqThreeValidCaseCount}{%
  \AblLoopCalc{0}{\RqThreeValidCaseCountFixed+\RqThreeValidCaseCountSymbolic}}
\newcommand{\RqThreeValidCaseCountFixed}{7\xspace}
\newcommand{\RqThreeValidCaseCountSymbolic}{7\xspace}
\newcommand{\RqThreeValidFixProved}{7\xspace}
\newcommand{\RqThreeValidFixMean}{1821.7\xspace}
\newcommand{\RqThreeValidFixMedian}{1741.7\xspace}
\newcommand{\RqThreeValidSymProved}{7\xspace}
\newcommand{\RqThreeValidSymMean}{1673.5\xspace}
\newcommand{\RqThreeValidSymMedian}{1471.2\xspace}

\newcommand{\RqThreeInvalidCaseCount}{%
  \AblLoopCalc{0}{\RqThreeInvalidCaseCountFixed+\RqThreeInvalidCaseCountSymbolic}}
\newcommand{\RqThreeInvalidCaseCountFixed}{7\xspace}
\newcommand{\RqThreeInvalidCaseCountSymbolic}{\RqThreeInvalidEvalCountSymbolic}
\newcommand{\RqThreeInvalidEvalCountSymbolic}{7\xspace}
\newcommand{\RqThreeInvalidFixRefuted}{6\xspace}
\newcommand{\RqThreeInvalidFixMean}{207.8\xspace}
\newcommand{\RqThreeInvalidFixMedian}{211.1\xspace}
\newcommand{\RqThreeInvalidSymRefuted}{7\xspace}
\newcommand{\RqThreeInvalidSymMean}{88.6\xspace}
\newcommand{\RqThreeInvalidSymMedian}{87.5\xspace}

\newcommand{\AblIntSum}[2]{\the\numexpr#1+#2\relax}
\newcommand{\AblIntDiff}[2]{\the\numexpr#1-#2\relax}
\newcommand{\AblMeanSeconds}[2]{\fpeval{round((#1)/(#2),1)}}
\newcommand{\AblSpeedup}[2]{\fpeval{round((#1)/(#2),1)}$\times$}
\newcommand{\AblCostReductionPercent}[2]{%
  \AblLoopCalc{1}{100*(1-(#2)/(#1))}\unskip\%\xspace}

\newcommand{\AblSymCountRaw}{30}
\newcommand{\AblFixCountRaw}{30}
\newcommand{\AblBaseSymSolvedRaw}{24}
\newcommand{\AblBaseFixSolvedRaw}{23}

\newcommand{\AblSymCount}{\AblSymCountRaw\xspace}
\newcommand{\AblFixCount}{\AblFixCountRaw\xspace}
\newcommand{\AblBaseSymSolved}{\AblBaseSymSolvedRaw\xspace}
\newcommand{\AblBaseFixSolved}{\AblBaseFixSolvedRaw\xspace}
\newcommand{\AblScafSymSolved}{\AblSymCountRaw\xspace}
\newcommand{\AblScafFixSolved}{\AblFixCountRaw\xspace}

\newcommand{\AblBaseCountRaw}{%
  \AblIntSum{\AblSymCountRaw}{\AblFixCountRaw}}
\newcommand{\AblBaseSolvedRaw}{%
  \AblIntSum{\AblBaseSymSolvedRaw}{\AblBaseFixSolvedRaw}}
\newcommand{\AblScafSolvedRaw}{%
  \AblIntSum{\AblSymCountRaw}{\AblFixCountRaw}}
\newcommand{\AblOnlyScafRaw}{%
  \AblIntDiff{\AblScafSolvedRaw}{\AblBaseSolvedRaw}}
\newcommand{\AblBaseCount}{\AblBaseCountRaw\xspace}
\newcommand{\AblBaseSolved}{\AblBaseSolvedRaw\xspace}
\newcommand{\AblScafSolved}{\AblScafSolvedRaw\xspace}

\newcommand{\AblPairSymSpeedup}{%
  \AblSpeedup{\AblPairSymBaseSecondsRaw}{\AblPairSymScafSecondsRaw}\xspace}
\newcommand{\AblPairFixSpeedup}{%
  \AblSpeedup{\AblPairFixBaseSecondsRaw}{\AblPairFixScafSecondsRaw}\xspace}
\newcommand{\AblPairSymBaseMean}{%
  \AblMeanSeconds{\AblPairSymBaseSecondsRaw}{\AblBaseSymSolvedRaw}\xspace}
\newcommand{\AblPairSymScafMean}{%
  \AblMeanSeconds{\AblPairSymScafSecondsRaw}{\AblBaseSymSolvedRaw}\xspace}
\newcommand{\AblPairFixBaseMean}{%
  \AblMeanSeconds{\AblPairFixBaseSecondsRaw}{\AblBaseFixSolvedRaw}\xspace}
\newcommand{\AblPairFixScafMean}{%
  \AblMeanSeconds{\AblPairFixScafSecondsRaw}{\AblBaseFixSolvedRaw}\xspace}

\newcommand{\AblPairBothSolvedRaw}{%
  \AblIntSum{\AblBaseSymSolvedRaw}{\AblBaseFixSolvedRaw}}
\newcommand{\AblPairSymBaseSecondsRaw}{78381.52}
\newcommand{\AblPairSymScafSecondsRaw}{18255.37}
\newcommand{\AblPairFixBaseSecondsRaw}{64207.49}
\newcommand{\AblPairFixScafSecondsRaw}{14589.76}
\newcommand{\AblPairBaseSecondsRaw}{%
  \fpeval{\AblPairSymBaseSecondsRaw+\AblPairFixBaseSecondsRaw}}
\newcommand{\AblPairScafSecondsRaw}{%
  \fpeval{\AblPairSymScafSecondsRaw+\AblPairFixScafSecondsRaw}}
\newcommand{\AblPairBaseMean}{%
  \AblMeanSeconds{\AblPairBaseSecondsRaw}{\AblPairBothSolvedRaw}\xspace}
\newcommand{\AblPairScafMean}{%
  \AblMeanSeconds{\AblPairScafSecondsRaw}{\AblPairBothSolvedRaw}\xspace}
\newcommand{\AblPairSpeedup}{%
  \AblSpeedup{\AblPairBaseSecondsRaw}{\AblPairScafSecondsRaw}\xspace}

\newcommand{\AblCexSymCountRaw}{30}
\newcommand{\AblCexFixCountRaw}{30}
\newcommand{\AblCexBaseSymRefutedRaw}{25}
\newcommand{\AblCexBaseFixRefutedRaw}{24}

\newcommand{\AblCexSymCount}{\AblCexSymCountRaw\xspace}
\newcommand{\AblCexFixCount}{\AblCexFixCountRaw\xspace}
\newcommand{\AblCexBaseSymRefuted}{\AblCexBaseSymRefutedRaw\xspace}
\newcommand{\AblCexBaseFixRefuted}{\AblCexBaseFixRefutedRaw\xspace}
\newcommand{\AblCexScafSymRefuted}{\AblCexSymCountRaw\xspace}
\newcommand{\AblCexScafFixRefuted}{\AblCexFixCountRaw\xspace}

\newcommand{\AblCexCountRaw}{%
  \AblIntSum{\AblCexSymCountRaw}{\AblCexFixCountRaw}}
\newcommand{\AblCexBaseRefutedRaw}{%
  \AblIntSum{\AblCexBaseSymRefutedRaw}{\AblCexBaseFixRefutedRaw}}
\newcommand{\AblCexScafRefutedRaw}{\AblCexCountRaw}
\newcommand{\AblCexOnlyScafRaw}{%
  \AblIntDiff{\AblCexScafRefutedRaw}{\AblCexBaseRefutedRaw}}
\newcommand{\AblOnlyScafTotalRaw}{%
  \AblIntSum{\AblOnlyScafRaw}{\AblCexOnlyScafRaw}}
\newcommand{\AblCexCount}{\AblCexCountRaw\xspace}
\newcommand{\AblCexBaseRefuted}{\AblCexBaseRefutedRaw\xspace}
\newcommand{\AblCexScafRefuted}{\AblCexScafRefutedRaw\xspace}

\newcommand{\AblCexPairSymBaseSecondsRaw}{22684.01}
\newcommand{\AblCexPairSymScafSecondsRaw}{1604}
\newcommand{\AblCexPairFixBaseSecondsRaw}{22416.91}
\newcommand{\AblCexPairFixScafSecondsRaw}{1392}
\newcommand{\AblCexPairBaseSecondsRaw}{%
  \fpeval{\AblCexPairSymBaseSecondsRaw+\AblCexPairFixBaseSecondsRaw}}
\newcommand{\AblCexPairScafSecondsRaw}{%
  \fpeval{\AblCexPairSymScafSecondsRaw+\AblCexPairFixScafSecondsRaw}}
\newcommand{\AblCexPairBothRaw}{\AblCexBaseRefutedRaw}
\newcommand{\AblCexPairSymSpeedup}{%
  \AblSpeedup{\AblCexPairSymBaseSecondsRaw}{\AblCexPairSymScafSecondsRaw}\xspace}
\newcommand{\AblCexPairFixSpeedup}{%
  \AblSpeedup{\AblCexPairFixBaseSecondsRaw}{\AblCexPairFixScafSecondsRaw}\xspace}
\newcommand{\AblCexPairSpeedup}{%
  \AblSpeedup{\AblCexPairBaseSecondsRaw}{\AblCexPairScafSecondsRaw}\xspace}
\newcommand{\AblCexPairBaseMean}{%
  \AblMeanSeconds{\AblCexPairBaseSecondsRaw}{\AblCexPairBothRaw}\xspace}
\newcommand{\AblCexPairScafMean}{%
  \AblMeanSeconds{\AblCexPairScafSecondsRaw}{\AblCexPairBothRaw}\xspace}
\newcommand{\AblCexPairSymBaseMean}{%
  \AblMeanSeconds{\AblCexPairSymBaseSecondsRaw}{\AblCexBaseSymRefutedRaw}\xspace}
\newcommand{\AblCexPairSymScafMean}{%
  \AblMeanSeconds{\AblCexPairSymScafSecondsRaw}{\AblCexBaseSymRefutedRaw}\xspace}
\newcommand{\AblCexPairFixBaseMean}{%
  \AblMeanSeconds{\AblCexPairFixBaseSecondsRaw}{\AblCexBaseFixRefutedRaw}\xspace}
\newcommand{\AblCexPairFixScafMean}{%
  \AblMeanSeconds{\AblCexPairFixScafSecondsRaw}{\AblCexBaseFixRefutedRaw}\xspace}

\newcommand{\AblCostSymBaseMean}{13.93}
\newcommand{\AblCostSymScafMean}{1.48}
\newcommand{\AblCostFixBaseMean}{12.49}
\newcommand{\AblCostFixScafMean}{1.45}
\newcommand{\AblCostBaseMean}{%
  \AblLoopCalc{2}{(\AblCostSymBaseMean*\AblBaseSymSolvedRaw
    +\AblCostFixBaseMean*\AblBaseFixSolvedRaw)/\AblPairBothSolvedRaw}}
\newcommand{\AblCostScafMean}{%
  \AblLoopCalc{2}{(\AblCostSymScafMean*\AblBaseSymSolvedRaw
    +\AblCostFixScafMean*\AblBaseFixSolvedRaw)/\AblPairBothSolvedRaw}}
\newcommand{\AblCostSymReduction}{%
  \AblCostReductionPercent{\AblCostSymBaseMean}{\AblCostSymScafMean}}
\newcommand{\AblCostFixReduction}{%
  \AblCostReductionPercent{\AblCostFixBaseMean}{\AblCostFixScafMean}}
\newcommand{\AblCostReduction}{%
  \AblCostReductionPercent{\AblCostBaseMean}{\AblCostScafMean}}

\newcommand{\AblCexCostSymBaseMean}{2.80}
\newcommand{\AblCexCostSymScafMean}{0.08}
\newcommand{\AblCexCostFixBaseMean}{3.52}
\newcommand{\AblCexCostFixScafMean}{0.08}
\newcommand{\AblCexCostBaseMean}{%
  \AblLoopCalc{2}{(\AblCexCostSymBaseMean*\AblCexBaseSymRefutedRaw
    +\AblCexCostFixBaseMean*\AblCexBaseFixRefutedRaw)/\AblCexPairBothRaw}}
\newcommand{\AblCexCostScafMean}{%
  \AblLoopCalc{2}{(\AblCexCostSymScafMean*\AblCexBaseSymRefutedRaw
    +\AblCexCostFixScafMean*\AblCexBaseFixRefutedRaw)/\AblCexPairBothRaw}}
\newcommand{\AblCexCostSymReduction}{%
  \AblCostReductionPercent{\AblCexCostSymBaseMean}{\AblCexCostSymScafMean}}
\newcommand{\AblCexCostFixReduction}{%
  \AblCostReductionPercent{\AblCexCostFixBaseMean}{\AblCexCostFixScafMean}}
\newcommand{\AblCexCostReduction}{%
  \AblCostReductionPercent{\AblCexCostBaseMean}{\AblCexCostScafMean}}

\ExplSyntaxOn
\cs_new_protected:Npn \AblLoopCalc #1#2
  {
    \group_begin:
    \cs_set:Npn \xspace { }
    \cs_set:Npn \ph ##1 { nan }
    \cs_set:Npn \AblLoopCalc ##1##2 { (##2) }
    \fp_trap:nn { invalid_operation } { none }
    \fp_trap:nn { division_by_zero } { none }
    \fp_set:Nn \l_tmpa_fp {#2}
    \bool_if:nTF
      {
        \fp_if_nan_p:n { \l_tmpa_fp } ||
        \fp_compare_p:n { abs(\l_tmpa_fp) = inf }
      }
      { \group_end: \ph{tbd} }
      {
        \use:x
          {
            \group_end:
            \fp_eval:n { round(\l_tmpa_fp,#1) }
            \exp_not:N \xspace
          }
      }
  }
\ExplSyntaxOff

\newcommand{\AblLoopPairSymCount}{\AblLoopBaseSymSolved}
\newcommand{\AblLoopPairFixCount}{\AblLoopBaseFixSolved}
\newcommand{\AblLoopPairCount}{%
  \AblLoopCalc{0}{\AblLoopPairSymCount+\AblLoopPairFixCount}}
\newcommand{\AblLoopCexPairSymCount}{\AblLoopCexBaseSymRefuted}
\newcommand{\AblLoopCexPairFixCount}{\AblLoopCexBaseFixRefuted}
\newcommand{\AblLoopCexPairCount}{%
  \AblLoopCalc{0}{\AblLoopCexPairSymCount+\AblLoopCexPairFixCount}}
\newcommand{\AblLoopCostSymCount}{\AblLoopPairSymCount}
\newcommand{\AblLoopCostFixCount}{\AblLoopPairFixCount}
\newcommand{\AblLoopCostCount}{%
  \AblLoopCalc{0}{\AblLoopCostSymCount+\AblLoopCostFixCount}}
\newcommand{\AblLoopCexCostSymCount}{\AblLoopCexPairSymCount}
\newcommand{\AblLoopCexCostFixCount}{\AblLoopCexPairFixCount}
\newcommand{\AblLoopCexCostCount}{%
  \AblLoopCalc{0}{\AblLoopCexCostSymCount+\AblLoopCexCostFixCount}}

\newcommand{\AblLoopSymCount}{\RqThreeValidCaseCountSymbolic}
\newcommand{\AblLoopBaseSymSolved}{6\xspace}
\newcommand{\AblLoopScafSymSolved}{\RqThreeValidSymProved}
\newcommand{\AblLoopPairSymBaseMean}{2784.5\xspace}
\newcommand{\AblLoopPairSymScafMean}{1446.6\xspace}
\newcommand{\AblLoopPairSymSpeedup}{%
  \AblLoopCalc{1}{\AblLoopPairSymBaseMean/\AblLoopPairSymScafMean}$\times$\xspace}
\newcommand{\AblLoopCostSymBaseMean}{12.06\xspace}
\newcommand{\AblLoopCostSymScafMean}{2.76\xspace}
\newcommand{\AblLoopCostSymReduction}{%
  \AblCostReductionPercent{\AblLoopCostSymBaseMean}{\AblLoopCostSymScafMean}}

\newcommand{\AblLoopFixCount}{\RqThreeValidCaseCountFixed}
\newcommand{\AblLoopBaseFixSolved}{6\xspace}
\newcommand{\AblLoopScafFixSolved}{\RqThreeValidFixProved}
\newcommand{\AblLoopPairFixBaseMean}{3042.1\xspace}
\newcommand{\AblLoopPairFixScafMean}{1603.4\xspace}
\newcommand{\AblLoopPairFixSpeedup}{%
  \AblLoopCalc{1}{\AblLoopPairFixBaseMean/\AblLoopPairFixScafMean}$\times$\xspace}
\newcommand{\AblLoopCostFixBaseMean}{13.35\xspace}
\newcommand{\AblLoopCostFixScafMean}{3.10\xspace}
\newcommand{\AblLoopCostFixReduction}{%
  \AblCostReductionPercent{\AblLoopCostFixBaseMean}{\AblLoopCostFixScafMean}}

\newcommand{\AblLoopCount}{%
  \AblLoopCalc{0}{\AblLoopSymCount+\AblLoopFixCount}}
\newcommand{\AblLoopBaseSolved}{%
  \AblLoopCalc{0}{\AblLoopBaseSymSolved+\AblLoopBaseFixSolved}}
\newcommand{\AblLoopScafSolved}{%
  \AblLoopCalc{0}{\AblLoopScafSymSolved+\AblLoopScafFixSolved}}
\newcommand{\AblLoopPairBaseMean}{%
  \AblLoopCalc{2}{(\AblLoopPairSymBaseMean*\AblLoopPairSymCount
    +\AblLoopPairFixBaseMean*\AblLoopPairFixCount)/\AblLoopPairCount}}
\newcommand{\AblLoopPairScafMean}{%
  \AblLoopCalc{2}{(\AblLoopPairSymScafMean*\AblLoopPairSymCount
    +\AblLoopPairFixScafMean*\AblLoopPairFixCount)/\AblLoopPairCount}}
\newcommand{\AblLoopPairSpeedup}{%
  \AblLoopCalc{1}{\AblLoopPairBaseMean/\AblLoopPairScafMean}$\times$\xspace}
\newcommand{\AblLoopCostBaseMean}{%
  \AblLoopCalc{2}{(\AblLoopCostSymBaseMean*\AblLoopCostSymCount
    +\AblLoopCostFixBaseMean*\AblLoopCostFixCount)/\AblLoopCostCount}}
\newcommand{\AblLoopCostScafMean}{%
  \AblLoopCalc{2}{(\AblLoopCostSymScafMean*\AblLoopCostSymCount
    +\AblLoopCostFixScafMean*\AblLoopCostFixCount)/\AblLoopCostCount}}
\newcommand{\AblLoopCostReduction}{%
  \AblCostReductionPercent{\AblLoopCostBaseMean}{\AblLoopCostScafMean}}

\newcommand{\AblLoopCexSymCount}{\RqThreeInvalidEvalCountSymbolic}
\newcommand{\AblLoopCexBaseSymRefuted}{7\xspace}
\newcommand{\AblLoopCexScafSymRefuted}{\RqThreeInvalidSymRefuted}
\newcommand{\AblLoopCexPairSymBaseMean}{697.2\xspace}
\newcommand{\AblLoopCexPairSymScafMean}{\RqThreeInvalidSymMean}
\newcommand{\AblLoopCexPairSymSpeedup}{%
  \AblLoopCalc{1}{\AblLoopCexPairSymBaseMean/\AblLoopCexPairSymScafMean}$\times$\xspace}
\newcommand{\AblLoopCexCostSymBaseMean}{2.20\xspace}
\newcommand{\AblLoopCexCostSymScafMean}{0.12\xspace}
\newcommand{\AblLoopCexCostSymReduction}{%
  \AblCostReductionPercent{\AblLoopCexCostSymBaseMean}{\AblLoopCexCostSymScafMean}}

\newcommand{\AblLoopCexFixCount}{\RqThreeInvalidCaseCountFixed}
\newcommand{\AblLoopCexBaseFixRefuted}{6\xspace}
\newcommand{\AblLoopCexScafFixRefuted}{\RqThreeInvalidFixRefuted}
\newcommand{\AblLoopCexPairFixBaseMean}{842.4\xspace}
\newcommand{\AblLoopCexPairFixScafMean}{\RqThreeInvalidFixMean}
\newcommand{\AblLoopCexPairFixSpeedup}{%
  \AblLoopCalc{1}{\AblLoopCexPairFixBaseMean/\AblLoopCexPairFixScafMean}$\times$\xspace}
\newcommand{\AblLoopCexCostFixBaseMean}{2.40\xspace}
\newcommand{\AblLoopCexCostFixScafMean}{0.37\xspace}
\newcommand{\AblLoopCexCostFixReduction}{%
  \AblCostReductionPercent{\AblLoopCexCostFixBaseMean}{\AblLoopCexCostFixScafMean}}

\newcommand{\AblLoopCexCount}{%
  \AblLoopCalc{0}{\AblLoopCexSymCount+\AblLoopCexFixCount}}
\newcommand{\AblLoopCexBaseRefuted}{%
  \AblLoopCalc{0}{\AblLoopCexBaseSymRefuted+\AblLoopCexBaseFixRefuted}}
\newcommand{\AblLoopCexScafRefuted}{%
  \AblLoopCalc{0}{\AblLoopCexScafSymRefuted+\AblLoopCexScafFixRefuted}}
\newcommand{\AblLoopCexPairBaseMean}{%
  \AblLoopCalc{2}{(\AblLoopCexPairSymBaseMean*\AblLoopCexPairSymCount
    +\AblLoopCexPairFixBaseMean*\AblLoopCexPairFixCount)/\AblLoopCexPairCount}}
\newcommand{\AblLoopCexPairScafMean}{%
  \AblLoopCalc{2}{(\AblLoopCexPairSymScafMean*\AblLoopCexPairSymCount
    +\AblLoopCexPairFixScafMean*\AblLoopCexPairFixCount)/\AblLoopCexPairCount}}
\newcommand{\AblLoopCexPairSpeedup}{%
  \AblLoopCalc{1}{\AblLoopCexPairBaseMean/\AblLoopCexPairScafMean}$\times$\xspace}
\newcommand{\AblLoopCexCostBaseMean}{%
  \AblLoopCalc{2}{(\AblLoopCexCostSymBaseMean*\AblLoopCexCostSymCount
    +\AblLoopCexCostFixBaseMean*\AblLoopCexCostFixCount)/\AblLoopCexCostCount}}
\newcommand{\AblLoopCexCostScafMean}{%
  \AblLoopCalc{2}{(\AblLoopCexCostSymScafMean*\AblLoopCexCostSymCount
    +\AblLoopCexCostFixScafMean*\AblLoopCexCostFixCount)/\AblLoopCexCostCount}}
\newcommand{\AblLoopCexCostReduction}{%
  \AblCostReductionPercent{\AblLoopCexCostBaseMean}{\AblLoopCexCostScafMean}}

